FlexFL: Flexible and Effective Fault Localization with Open-Source Large Language Models

Due to the impressive code comprehension ability of Large Language Models (LLMs), a few studies have proposed to leverage LLMs to locate bugs, i.e., LLM-based FL, and demonstrated promising performance. However, first, these methods are limited in flexibility. They rely on bug-triggering test cases to perform FL and cannot make use of other available bug-related information, e.g., bug reports. Second, they are built upon proprietary LLMs, which are, although powerful, confronted with risks in data privacy. To address these limitations, we propose a novel LLM-based FL framework named FlexFL, which can flexibly leverage different types of bug-related information and effectively work with open-source LLMs. FlexFL is composed of two stages. In the first stage, FlexFL reduces the search space of buggy code using state-of-the-art FL techniques of different families and provides a candidate list of bug-related methods. In the second stage, FlexFL leverages LLMs to delve deeper to double-check the code snippets of methods suggested by the first stage and refine fault localization results. In each stage, FlexFL constructs agents based on open-source LLMs, which share the same pipeline that does not postulate any type of bug-related information and can interact with function calls without the out-of-the-box capability. Extensive experimental results on Defects4J demonstrate that FlexFL outperforms the baselines and can work with different open-source LLMs. Specifically, FlexFL with a lightweight open-source LLM Llama3-8B can locate 42 and 63 more bugs than two state-of-the-art LLM-based FL approaches AutoFL and AgentFL that both use GPT-3.5.

==> sections/abstract_conference.tex <==
\maketitle

\begin{abstract}
Fault localization (FL) targets identifying bug locations within a software system, which can enhance debugging efficiency and improve software quality. 
Due to the impressive code comprehension ability of Large Language Models (LLMs), a few studies have proposed to leverage LLMs to locate bugs, i.e., LLM-based FL, and demonstrated promising performance.
However, first, these methods are limited in flexibility. They rely on bug-triggering test cases to perform FL and cannot make use of other available bug-related information, e.g., bug reports.
Second, they are built upon proprietary LLMs, which are, although powerful, confronted with risks in data privacy.
To address these limitations, we propose a novel LLM-based FL framework named \name, which can flexibly leverage different types of bug-related information and effectively work with open-source LLMs.
\name is composed of two stages.
In the first stage, \name reduces the search space of buggy code using state-of-the-art FL techniques of different families and provides a candidate list of bug-related methods.
In the second stage, \name leverages LLMs to delve deeper to double-check the code snippets of methods suggested by the first stage and refine fault localization results.
In each stage, \name constructs agents based on open-source LLMs, which share the same pipeline that does not postulate any type of bug-related information and can interact with function calls without out-of-the-box features.
% and then leverages LLMs to delve deeper to double-check the code snippets of suspicious methods and refine fault localizations in the second stage.
% It simulates the developers' debugging process and complements traditional FL techniques and LLMs to make traditional techniques more accurate and LLMs more practical. 
% We evaluate our \name on Defects4j.
Extensive experimental results on Defects4J demonstrate that the \name can outperform the baselines and work with different open-source LLMs.
Specifically, \name with a lightweight open-source LLM Llama3-8B can locate 42 more bugs than the state-of-the-art LLM-based FL approach AutoFL that uses GPT-3.5. 
In addition, \name can localize 93 bugs that cannot be localized by non-LLM-based FL techniques at the top 1.
% Furthermore, we also conduct experiments on the GHRB dataset to mitigate potential data leakage, and evaluation results show that \name achieves comparable performance on both datasets, suggesting that \name’s performance is not solely due to model memorization.

%evaluation
\end{abstract}

% \begin{IEEEkeywords}
% Fault Localization, Large Language Model, Language Agent.
% \end{IEEEkeywords}

